Decouple Learning for Parameterized Image Operators

Many different deep networks have been used to approximate, accelerate or improve traditional image operators, such as image smoothing, super-resolution and denoising. Among these traditional operators, many contain parameters which need to be tweaked to obtain the satisfactory results, which we refer to as "parameterized image operators". However, most existing deep networks trained for these operators are only designed for one specific parameter configuration, which does not meet the needs of real scenarios that usually require flexible parameters settings. To overcome this limitation, we propose a new decouple learning algorithm to learn from the operator parameters to dynamically adjust the weights of a deep network for image operators, denoted as the base network. The learned algorithm is formed as another network, namely the weight learning network, which can be end-to-end jointly trained with the base network. Experiments demonstrate that the proposed framework can be successfully applied to many traditional parameterized image operators. We provide more analysis to better understand the proposed framework, which may inspire more promising research in this direction. Our codes and models have been released in https://github.com/fqnchina/DecoupleLearning

==> figure1.tex <==
\setlength{\tabcolsep}{1pt}
% \renewcommand{\arraystretch}{1}
\begin{figure*}[t]
\begin{center}

\begin{tabular}{cccccc}


$\lambda$ &0.002 & 0.004 & 0.020 & 0.093 & 0.200
\\
\raisebox{2.0\height}{\rotatebox[origin=c]{90}{\footnotesize{{GT}}}}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-000200.png}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-000431.png}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-002000.png}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-009283.png}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-020000.png}
\\

\raisebox{1.65\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-000200-predict.png}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-000431-predict.png}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-002000-predict.png}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-009283-predict.png}
&\includegraphics[width=2.20cm]{./L0smooth_random/2011_006853-L0smooth-020000-predict.png}
\\


$\lambda$ &0.100 & 0.215 & 1.000 & 4.641 & 10.00
\\
\raisebox{2.0\height}{\rotatebox[origin=c]{90}{\footnotesize{{GT}}}}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-010000.png}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-021544.png}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-100000.png}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-464159.png}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-1000000.png}
\\

\raisebox{1.5\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-010000-predict.png}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-021544-predict.png}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-100000-predict.png}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-464159-predict.png}
&\includegraphics[width=2.20cm]{./WLS_random/2012_003923-WLS-1000000-predict.png}
\\

$\lambda$ &0.002 & 0.004 & 0.010 & 0.022 & 0.050
\\

\raisebox{2.0\height}{\rotatebox[origin=c]{90}{\footnotesize{{GT}}}}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-000200.png}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-000447.png}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-001000.png}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-002236.png}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-005000.png}
\\

\raisebox{1.5\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-000200-predict.png}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-000447-predict.png}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-001000-predict.png}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-002236-predict.png}
&\includegraphics[width=2.20cm]{./RTV_random/2007_000480-RTV-005000-predict.png}
\\


\end{tabular}

\end{center}
\caption{Visual examples produced by our framework trained on continuous parameter settings of $L_0$ \cite{xu2011image} (top), WLS \cite{farbman2008edge} (middle) and RTV \cite{xu2012structure} (bottom) filters independently. Note all the smooth images for one filter are generated by a single network.}
\label{figure:1}
\end{figure*} 


==> figure2.tex <==
\setlength{\tabcolsep}{1pt}
% \vspace{-6mm}
\begin{figure*}[t]
\begin{center}

\begin{tabular}{cccccc}
$s$ &2.0 & 2.5 & 3.0 & 3.5 & 4.0
\\

\raisebox{2.3\height}{\rotatebox[origin=c]{90}{\footnotesize{{Input}}}}
&\includegraphics[width=2.20cm]{foreman-SR-20-ycbcr.png}
&\includegraphics[width=2.20cm]{foreman-SR-25-ycbcr.png}
&\includegraphics[width=2.20cm]{foreman-SR-30-ycbcr.png}
&\includegraphics[width=2.20cm]{foreman-SR-35-ycbcr.png}
&\includegraphics[width=2.20cm]{foreman-SR-40-ycbcr.png}
\\
\raisebox{2.0\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{foreman-SR-20-predict-color.png}
&\includegraphics[width=2.20cm]{foreman-SR-25-predict-color.png}
&\includegraphics[width=2.20cm]{foreman-SR-30-predict-color.png}
&\includegraphics[width=2.20cm]{foreman-SR-35-predict-color.png}
&\includegraphics[width=2.20cm]{foreman-SR-40-predict-color.png}
\\
&(32.86dB/0.958)&(30.96dB/0.939)&(29.88dB/0.923)&(29.01dB/0.907)&(28.08dB/0.888)\\

\raisebox{1.6\height}{\rotatebox[origin=c]{90}{\footnotesize{{Input}}}}
&\includegraphics[width=2.20cm]{monarch-SR-20-ycbcr.png}
&\includegraphics[width=2.20cm]{monarch-SR-25-ycbcr.png}
&\includegraphics[width=2.20cm]{monarch-SR-30-ycbcr.png}
&\includegraphics[width=2.20cm]{monarch-SR-35-ycbcr.png}
&\includegraphics[width=2.20cm]{monarch-SR-40-ycbcr.png}
\\
\raisebox{1.6\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{monarch-SR-20-predict-color.png}
&\includegraphics[width=2.20cm]{monarch-SR-25-predict-color.png}
&\includegraphics[width=2.20cm]{monarch-SR-30-predict-color.png}
&\includegraphics[width=2.20cm]{monarch-SR-35-predict-color.png}
&\includegraphics[width=2.20cm]{monarch-SR-40-predict-color.png}
\\
&(34.74dB/0.969)&(33.23dB/0.959)&(31.91dB/0.948)&(30.72dB/0.935)&(29.49dB/0.920)\\

$\sigma$ & 0.033 & 0.069 & 0.100 & 0.208 & 0.300\\

\raisebox{2.1\height}{\rotatebox[origin=c]{90}{\footnotesize{{Input}}}}
&\includegraphics[width=2.20cm]{2010_005426-noise-003333.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-006934.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-010000.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-020801.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-030000.png}
\\
\raisebox{2.0\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{2010_005426-noise-003333-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-006934-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-010000-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-020801-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-030000-predict.png}
\\
&(35.69dB/0.956)&(34.22dB/0.941)&(32.59dB/0.922)&(29.31dB/0.876)&(27.23dB/0.838)\\

\end{tabular}

\end{center}
\vspace{-6mm}
\caption{Qualitative evaluation of our network trained with random scales for the image super resolution and denoising task. As can be seen, our network is able to compensate the lost details well for all the different degrees of corrupted images.}
\label{figure:2}
\vspace{-6mm}
\end{figure*} 

==> figure3.tex <==
\setlength{\tabcolsep}{1pt}
\begin{figure*}[h]
\begin{center}

\begin{tabular}{cccccc}
$\sigma$ & 0.033 & 0.069 & 0.100 & 0.208 & 0.300
\\

\raisebox{3.6\height}{\rotatebox[origin=c]{90}{\footnotesize{{Input}}}}
&\includegraphics[width=2.20cm]{2008_006815-noise-003333.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-006934.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-010000.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-020801.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-030000.png}
\\
\raisebox{3.35\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{2008_006815-noise-003333-predict.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-006934-predict.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-010000-predict.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-020801-predict.png}
&\includegraphics[width=2.20cm]{2008_006815-noise-030000-predict.png}
\\
&(33.58dB/0.955)&(31.10dB/0.919)&(29.62dB/0.891)&(26.44dB/0.801)&(24.76dB/0.745)\\

\raisebox{2.1\height}{\rotatebox[origin=c]{90}{\footnotesize{{Input}}}}
&\includegraphics[width=2.20cm]{2010_005426-noise-003333.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-006934.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-010000.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-020801.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-030000.png}
\\
\raisebox{2.0\height}{\rotatebox[origin=c]{90}{\footnotesize{{Ours}}}}
&\includegraphics[width=2.20cm]{2010_005426-noise-003333-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-006934-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-010000-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-020801-predict.png}
&\includegraphics[width=2.20cm]{2010_005426-noise-030000-predict.png}
\\
&(35.69dB/0.956)&(34.22dB/0.941)&(32.59dB/0.922)&(29.31dB/0.876)&(27.23dB/0.838)\\

\end{tabular}

\end{center}
\vspace{-4mm}
\caption{Demonstration of the value of our network on the denoising task. Despite different degrees of gaussian noise, our single network jointly trained on random parameters is able to remove them all well.}
\label{figure:3}
\end{figure*} 
